Software Verification with PDR: Implementation and Empirical Evaluation of the State of the Art

Property-directed reachability (PDR) is a SAT/SMT-based reachability algorithm that incrementally constructs inductive invariants. After it was successfully applied to hardware model checking, several adaptations to software model checking have been proposed. We contribute a replicable and thorough comparative evaluation of the state of the art: We (1) implemented a standalone PDR algorithm and, as improvement, a PDR-based auxiliary-invariant generator for k-induction, and (2) performed an experimental study on the largest publicly available benchmark set of C verification tasks, in which we explore the effectiveness and efficiency of software verification with PDR. The main contribution of our work is to establish a reproducible baseline for ongoing research in the area by providing a well-engineered reference implementation and an experimental evaluation of the existing techniques.

==> evaluation/plot-defs.tex <==
%
%
\makeatletter
\pgfdeclareplotmark{halfsquarent*}{%
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{-\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{-\pgfplotmarksize}{\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{-\pgfplotmarksize}}%
  \pgfusepathqfill
  \ifx\pgf@mark@color@none\pgf@mark@color
  \else
    \pgfscope
      \pgf@set@mark@color
      \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}%
      \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}%
      \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{\pgfplotmarksize}}%
      \pgfpathlineto{\pgfqpoint{-\pgfplotmarksize}{\pgfplotmarksize}}%
      \pgfusepathqfill
    \endpgfscope
  \fi
  \pgfpathmoveto{\pgfqpoint{\pgfplotmarksize}{-\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{-\pgfplotmarksize}{\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{-\pgfplotmarksize}{-\pgfplotmarksize}}%
  \pgfpathclose
  \pgfusepathqstroke
}
\makeatother

\pgfplotsset{
  %
  quantile plot/.style={
    width=.85\linewidth,
    scale only axis,
    %
    /pgfplots/table/x index=0,
    /pgfplots/table/y index=3,
    /pgfplots/table/header=false,
    %
    ylabel shift=-1em,
    ticklabel style={font={\smaller}},
    %
    ymin=1,
    ymax=1000,
    %
    legend cell align={left},
    legend style={at={(0,1)}, anchor=north west, outer xsep=4pt, outer ysep=4pt, inner ysep=0pt, fill=none, font={\smaller}},
    legend columns=1,
    mark size=3pt,
    cycle multiindex list={
      orange, red, blue, purple, cyan, brown, black\nextlist
      mark=*, mark=halfsquare*, mark=triangle*, mark=triangle*, mark=halfsquarent*, mark=halfdiamond*, mark=halfcircle*\nextlist
      mark options={solid}, mark options={solid}, mark options={solid}, mark options={solid,rotate=180}, mark options={solid}, mark options={solid}, mark options={solid}, mark options={solid}\nextlist
      solid, densely dashed, densely dashdotdotted, densely dotted},
  },
  every axis plot/.append style={thick},
  %
  %
  %
  %
  %
  split quantile plot/.style={
    xtick align=inside,
    every axis y label/.append style={at=(ticklabel cs:0.4)},
  },
  split quantile plot top/.style={
    quantile plot,
    width=.85\linewidth,
    height=.75\linewidth,
    xmajorticks=false,
    xminorticks=false,
    xlabel=,
  },
  split quantile plot bottom/.style={
    quantile plot,
    ylabel=,
    ymin=0,ymax=1,
    restrict y to domain=0:1,
    width=.85\linewidth,
    height=.10\linewidth,
    ytick={0},
    xtick pos=left,
  },
}

  \pgfplotsset{quantile plot/.append style={
      ylabel=CPU time (\second),
      xlabel=Accumulated score,
    },
  }

\newenvironment{pgfplot}{
  \begin{minipage}{252pt}
  \begin{tikzpicture}
}{
  \end{tikzpicture}
  \end{minipage}
}

\newcommand\addgraph[3][]{{
  \newcommand\csvfile{\plotpath/\detokenize{#3}}
  \IfFileExists\csvfile{
    \addplot+[#1] table {\csvfile}; \addlegendentry{#2}
  }{
    \addplot[#1] coordinates {};
  }
}}

\newcommand{\modulo}[2]{\fpeval{trunc(#1-(#2*trunc(#1/#2,0)),0)}}
\newcommand{\offset}[2]{\fpeval{#2-(\modulo{#1}{#2})}}

